Neural Network Constraints on the Cosmic-Ray Ionization Rate and Other Physical Conditions in NGC 253 with ALCHEMI Measurements of HCN and HNC

We use a neural network model and ALMA observations of HCN and HNC to constrain the physical conditions, most notably the cosmic-ray ionization rate (CRIR, zeta), in the Central Molecular Zone (CMZ) of the starburst galaxy NGC 253. Using output from the chemical code UCLCHEM, we train a neural network model to emulate UCLCHEM and derive HCN and HNC molecular abundances from a given set of physical conditions. We combine the neural network with radiative transfer modeling to generate modeled integrated intensities, which we compare to measurements of HCN and HNC from the ALMA Large Program ALCHEMI. Using a Bayesian nested sampling framework, we constrain the CRIR, molecular gas volume and column densities, kinetic temperature, and beam-filling factor across NGC 253's CMZ. The neural network model successfully recovers UCLCHEM molecular abundances with about 3 percent error and, when used with our Bayesian inference algorithm, increases the parameter inference speed tenfold. We create images of these physical parameters across NGC 253's CMZ at 50 pc resolution and find that the CRIR, in addition to the other gas parameters, is spatially variable with zeta a few times 10^{14} s^{-1} at greater than 100 pc from the nucleus, increasing to zeta greater than 10^{-13} s^{-1} at its center. These inferred CRIRs are consistent within 1 dex with theoretical predictions based on non-thermal emission. Additionally, the high CRIRs estimated in NGC 253's CMZ can be explained by the large number of cosmic-ray-producing sources as well as a potential suppression of cosmic-ray diffusion near their injection sites.

==> Notes.tex <==
\subsection{Old Versus New Rates -- H$_{3}$O$^{+}$}

\begin{figure*}
%\hspace{-12mm}
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=3in, height=3in, trim = 0mm 2mm 5mm 0mm]{h3opSO_corner26_oldRates.pdf}
  %\vspace{-5mm}
  \caption{}
  \label{fig:h3opSO_reg26_oldRates}
\end{subfigure}%
%\hspace{-40mm}
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=3in, height=3in, trim = 0mm 2mm 5mm 0mm]{h3opSO_corner26_newRates.pdf}
  %\vspace{-5mm}
  \caption{}
  \label{fig:h3opSO_reg26_newRates}
\end{subfigure}%
\caption{\texttt{UltraNest} inferencing results derived from H$_{3}$O$^{+}$ and SO data for region 26 using old (left) versus new(right) H$_{3}$O$^{+}$ collisional excitation rates.}
\label{fig:reg26Rates}
\end{figure*}


\begin{figure*}
%\hspace{-12mm}
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=3in, height=3in, trim = 5mm 2mm 5mm 0mm]{h3opSO_corner53_oldRates.pdf}
  %\vspace{-5mm}
  \caption{}
  \label{fig:h3opSO_reg53_oldRates}
\end{subfigure}%
%\hspace{-40mm}
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=3in, height=3in, trim = 5mm 2mm 10mm 0mm]{h3opSO_corner53_newRates.pdf}
  %\vspace{-5mm}
  \caption{}
  \label{fig:h3opSO_reg53_newRates}
\end{subfigure}%
\caption{Same as in Figure \ref{fig:reg26Rates} but for region 53.}
\label{fig:reg53Rates}
\end{figure*}


\begin{figure*}
%\hspace{-12mm}
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=3in, height=3in, trim = 0mm 2mm 5mm 0mm]{h3op_SO_corner86_oldRates.pdf}
  %\vspace{-5mm}
  \caption{}
  \label{fig:h3opSO_reg86_oldRates}
\end{subfigure}%
%\hspace{-40mm}
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=3in, height=3in, trim = 0mm 2mm 5mm 0mm]{h3opSO_corner86_newRates.pdf}
  %\vspace{-5mm}
  \caption{}
  \label{fig:h3opSO_reg86_newRates}
\end{subfigure}%
\caption{Same as in Figure \ref{fig:reg26Rates} but for region 86.}
\label{fig:reg86Rates}
\end{figure*}


\begin{itemize}
    \item CR generation by SNRs \citep{Phan2024} and other sources 
    \begin{itemize}
        \item Note that they assume that x-ray ionization is unimportant and that the XRIR in starbursts is $\zeta_{x-ray} \lesssim 10^{-17}$\,s$^{-1}$.  Furthermore, I posed the question to Serena (why do we not model x-ray ionization), who said that from the point of view of UCLCHEM there is no difference between a CR-induced and an x-ray-induced reaction.  She thought that the high TK associated with high x-ray fluxes argued against a high concentration of x-rays for the regions we study, but has not yet defined what "high Tk" is.
        \item refer back to Discussion of \cite{Behrens2022} where we talk about CRIR estimated from supernova explosion rates
    \end{itemize}
\end{itemize}


\begin{itemize}
    \item cosmic-ray buildup in high-density regions explored by \cite{Semenov2021}
    \begin{itemize}
        \item explore isotropic diffusion for CR propogation where diffusion coefficient is suppressed near injection sites in star-forming regions
        \item CRs mostly accelerated by shocks around supernova remnants, but also possibly from stellar wind shocks
        \item average diffusion coefficient $\kappa_{\text{CR}}$ for MW is $\kappa_{\text{CR}}\sim10^{28}$\,cm$^{2}$\,s$^{-1}$
        \item theoretical backing: in environments with strong shocks, most assumptions regarding CR propagation are violated---CR current is much higher, resulting in the excitation of nonresonant modes and plasma instabilities---background magnetic field is amplified, leading to what is called the Bohn diffusion regime, where the diffusion coefficient is smaller by a factor of $\sim10^6$
        \item observational backing: modeling of nearby Galactic molecular clouds and supernova remnants has indicated that $\kappa$ is suppressed by a factor of 10--100 in star-forming regions; region affected by suppressed diffusion is a few tens of parsecs $\lesssim d \lesssim 50$\,pc
        \item model assumes 20\% of Type II supernova energy is injected as CRs---canonical MW values is 10\% \citep[][such as used in]{Phan2024}, but \cite{Semenov2021} assumes most SNe explode in regions that already contain CRs accelerated by stellar wind shocks or previous SNe (probably a good assumption based on UA97 data), so CRs produced before the SNa can be reaccelerated, leading to higher energy efficiency than 10\%
        \item model allows $\kappa$ to vary---in average ISM and halo, $\kappa_{\text{CR},0}=10^{28}$\,cm$^{2}$\,s$^{-1}$, but in regions with active SNe, the turbulent diffusivity $\kappa_{\text{turb}}$ is 200--1000 times smaller than $\kappa_{\text{CR},0}$
        \item diffusion is only suppressed in areas where $t_{\text{age}} < t_{\text{SN}} = 40$\,Myr, which is equivalent to timescale for shocks and superbubbles to be sustained for a single-age population of stars
        \item for $\kappa < 10^{26}$\,cm$^{2}$\,s$^{-1}$, diffusion is saturated, so timescales for CRs remaining in one location is controlled by the liftime of the supernova bubbles
        \item results
        \begin{itemize}
            \item CR feedback results in fewer dense, star-forming clumps, and this is only enhanced when CR diffusion is considered
            \item cosmic-ray pressure is significantly enhanced, especially in the galaxy center, when CR diffusion suppression is applied--this pressure can both stop dense gas clumps from forming on smaller scales as well as prevent the fragmentation of the gaseous galaxy disk, providing disk stability and support (this usually happens after SNa explosions stop and CRs escape into ISM)
            \item for galaxies with low gas masses, CR feedback can regulate galaxy evolution by driving galactic winds; for high-mass galaxies, CR feedback suppresses both disk fragmentation and the formation of dense gas structures
            \item galaxies with higher gas fractions (40\% versus 20\% seem to be more susceptible to changes in ISM structure as a result of CR diffusion suppression and CR pressure makes up a larger portion of the total pressure budget 
            \item SFR reduced by a factor of $\sim$3--4 when CR diffusion is suppressed
        \end{itemize}
    \end{itemize}
\end{itemize}
